DP-REC: Private & Communication-Efficient Federated Learning

Privacy and communication efficiency are important challenges in federated training of neural networks, and combining them is still an open problem. In this work, we develop a method that unifies highly compressed communication and differential privacy (DP). We introduce a compression technique based on Relative Entropy Coding (REC) to the federated setting. With a minor modification to REC, we obtain a provably differentially private learning algorithm, DP-REC, and show how to compute its privacy guarantees. Our experiments demonstrate that DP-REC drastically reduces communication costs while providing privacy guarantees comparable to the state-of-the-art.

==> ICLR 2022/sections/conclusion.tex <==
\section{Conclusion}
With \ourmethod{}, we formalized the intuitive notion that $\varepsilon,\delta$ differentially private messages necessarily contain a small amount of information and can therefore be compressed significantly. A bound on the R\'enyi divergence between the server-side prior $p$ and the locally optimized $q$ implies a small message size for \rec{}, elegantly tying together DP and communication efficiency for federated learning. The nature of our bound in Theorem \ref{the:Theorem1} reveals the flipside of \ourmethod{}. As opposed to the standard Gaussian mechanism in central DP, it requires stronger clipping, effectively reducing the utility of models trained with \ourmethod{} for a given privacy budget. Our experiments with the StackOverflow dataset show that these limitations can be mitigated by the stronger privacy amplification in situations with large numbers of clients. Contrary to intuition, spending more bits to communicate updates from clients to the server cannot recover this utility as the necessary information is lost in clipping, \emph{i.e.}, before forming the importance sampling distribution $\tilde{q}$.

There are several important directions left for future work. The first would be to investigate the convergence of \ourmethod{}. Intuitively, we can expect the algorithm to be convergent if \dpfedavg{} is convergent. The main difference of \ourmethod{} is that the gradient is sampled using importance weights rather than the true Gaussian probabilities. Asymptotically, these two distributions should be close, and the bias of the compressed gradients would be bounded by a small value (as discussed in Section~\ref{sec:privacy_analysis}). Empirically, we observe no issues with convergence. The second would be to investigate secure shuffling, similarly to \citet{girgis2020shuffled} as a way to amplify our privacy further; this can lead to less aggressive clipping and thus improved performance for a given privacy budget.

We expect our work to have an overall beneficial societal impact through its main contributions of communication reduction and differential privacy. One potential concern worth mentioning is the interplay between differential privacy and fairness in FL, an actively researched open problem. \citet{bagdasaryan2019differential} demonstrate that DP training can have a disproportionate effect on underrepresented and more complex sub-populations, resulting in a disparate accuracy reduction. At the same time, \citet{hooker2020characterising} showed that compression of models can have negative impacts by amplifying biases. In the context of FL, compression is performed on model updates instead of a final model, therefore requiring further research on its influence on bias amplification.

==> ICLR 2022/sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}
We evaluate \ourmethod{} on several non-i.i.d. FL tasks that provide client-level privacy guarantees: image classification on a non-i.i.d. split of MNIST~\citep{lecun1998gradient} into $100$ clients and FEMNIST~\citep{caldas2018leaf} into $3.5$k clients, along with next character prediction on the Shakespeare dataset~\citep{caldas2018leaf} with LSTMs~\citep{hochreiter1997long} and $660$ clients as well as tag prediction on the StackOverflow (SO-LR) dataset~\citep{stackoverflow2019} with a logistic regression model~\citep{kairouz2021distributed} and $342477$ clients. For baselines, we consider \dpfedavg{} as the gold standard without compression and \ddgauss{} as a baseline that involves parameter quantization. Both of these methods target central DP guarantees and employ secure aggregation. All exeriments were implemented in PyTorch \citep{NEURIPS2019_9015}. We provide experimental details in Appendix \ref{sec:AppExpDetails}.

\subsection{Results and discussion}
\label{sec:experiments_privacy}
We plot the global model accuracy for different privacy budgets $\varepsilon$ as a function of the total communication cost in Figure~\ref{fig:comm_vs_acc}; this highlights how efficiently each method spends bits of communication in order to reach a target accuracy. Due to the substantial compression by \ourmethod{} relative to the baselines, we use \emph{log-scale} for the x-axis of communication costs. Additionally, Figure~\ref{fig:priv_vs_acc} in Appendix~\ref{sec:AppAdditionalResults} shows the accuracy achieved as a function of the privacy budget $\varepsilon$; this highlights how efficiently each method spends its privacy budget in order to reach a specific target accuracy. Note that in certain cases the training is stopped before convergence, due to exhausted privacy budget. 

In Table~\ref{tab:acc_comm_res}, we report the final model performance and total communication costs for different privacy budgets. It should be mentioned that the evaluation loop for StackOverflow is prohibitively expensive to be done in each round due to having ${\scriptscriptstyle~^\sim}1.6$M datapoints. We thus pick $10$k random datapoints for evaluation during training to plot the learning curves (not necessarily the same for each run), following~\citep{reddi2020adaptive}. The numbers in Table~\ref{tab:acc_comm_res} refer to the model performance at the end of training, where we evaluate on the entire test set for \dpfedavg{} and \ourmethod{}. For \ddgauss{}, since \citet{kairouz2021distributed} do not report the model performance on the full test set, we use the numbers shown at the end of their plot. Finally, results for some settings are omitted because of either (i) convergence issues for stricter privacy budgets (a typical phenomenon for $\varepsilon < 1$ on smaller federations); (ii) not being reported by the related work we compare with; or (iii) not being necessary in light of sufficient performance under better privacy guarantees (e.g., on StackOverflow).

\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3pt}
\caption{Performance ($\pm$ standard error obtained via multiple runs) and total communication (in GB),  achieved for different privacy guarantees $\varepsilon$. Results for \ddgauss{} (marked \ddg{$x$} for $x$ bits) are taken from~\citep{kairouz2021distributed}, which uses a slightly smaller version of the FEMNIST dataset ($3.4k$ clients instead of $3.5k$). }
\resizebox{0.4\textwidth}{!}{ 
\begin{tabular}[t]{lcc}
\toprule
{\bf MNIST} & \dpfedavg{} & \ourmethod{} \\
\midrule
Acc. ($\varepsilon\!=\!3$) & $82.1\pm0.8$ & $69.5\pm1.5$ \\
Acc. ($\varepsilon\!=\!6$) & $90.0\pm0.4$ & $83.7\pm0.6$ \\
\emph{Comm.} & \emph{43} & \emph{0.01} \\
\end{tabular}}
~
\resizebox{0.55\textwidth}{!}{ 
\begin{tabular}[t]{lcccc}
\toprule
{\bf FEMNIST} & \dpfedavg{} & \ddg{16} & \ddg{12} & \ourmethod{} \\
\midrule
Acc. ($\varepsilon\!=\!1$) & $66.0\pm0.2$ & -- & -- & $59.7\pm0.3$ \\
Acc. ($\varepsilon\!=\!3$) & $74.6\pm0.1$ & ${\scriptscriptstyle~^\sim}72$ & ${\scriptscriptstyle~^\sim}25$ & $67.1\pm0.2$ \\
Acc. ($\varepsilon\!=\!6$) & $75.6\pm0.1$ & ${\scriptscriptstyle~^\sim}77$ & ${\scriptscriptstyle~^\sim}71$ & $69.2\pm0.3$ \\
\emph{Comm.} & \emph{259} & \emph{194} & \emph{178} & \emph{14.2} \\
\end{tabular}}
\resizebox{0.4\textwidth}{!}{ 
\begin{tabular}[t]{lcc}
\toprule
{\bf Shakespeare} & \dpfedavg{} & \ourmethod{} \\
\midrule
Acc. ($\varepsilon\!=\!3$) & $39.0\pm0.1$ & $29.2\pm0.2$ \\
\emph{Comm.} & \emph{81} & \emph{0.1} \\
\bottomrule
\end{tabular}
}
\resizebox{0.55\textwidth}{!}{ 
\begin{tabular}[t]{lcccc}
\toprule
{\bf SO LR} & \dpfedavg{} & \ddg{16} & \ddg{12} & \ourmethod{} \\
\midrule
R@5 ($\varepsilon\!=\!1)$ & $19.3\pm0.0$ & ${\scriptscriptstyle~^\sim}14$ & ${\scriptscriptstyle~^\sim}10$ & $18.4\pm0.7$ \\
\emph{Comm.} & \emph{3356} & \emph{2517} & \emph{2307} & \emph{32} \\
\bottomrule
\end{tabular}}
\label{tab:acc_comm_res}
\end{table*}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.41\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mnist_gb_acc_vf.png}
        \caption{MNIST}
        \label{fig:mnist_communication_accuracy}
    \end{subfigure}%
    \begin{subfigure}{0.41\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/femnist_gb_acc_vf.png}
        \caption{FEMNIST}
        \label{fig:femnist_communication_accuracy}
    \end{subfigure}\\
    \begin{subfigure}{0.41\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/shakespeare_gb_acc_vf.png}
        \caption{Shakespeare}
        \label{fig:shakespeare_communication_accuracy}
    \end{subfigure}%
    \begin{subfigure}{0.41\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/gb_acc_SO_v2.png}
        \caption{StackOverflow}
        \label{fig:stackoverflow_communication_accuracy}
    \end{subfigure}
    \caption{Test accuracy (\%) with $\pm 1$ standard error as a function of communication (in GB, in \emph{log-scale}). For StackOverflow, we report compression at the end of training, as the learning curves are based on different subsets of the validation set.} \label{fig:comm_vs_acc}
\end{figure}

Observing the experimental results, we clearly see the trade-offs. \ourmethod{} can drastically reduce the \emph{total communication costs} (download and upload) of federated training depending on the subsampling rate and amount of clients in a federation. In some cases, we can get extreme reduction, such as MNIST with $4300$x compression (end-points of curves on Figure~\ref{fig:comm_vs_acc}). Otherwise, the reduction is still several orders of magnitude ($105$x for SO-LR and $18$x on FEMNIST). 
Nevertheless, \dpfedavg{} and \ddgauss{} (depending on the task) can reach better model performance for a given privacy budget. This is primarily due to two reasons. Firstly, both \dpfedavg{} and \ddgauss{} add noise calibrated to the number of clients in a given round to get a central DP guarantee on the aggregate; in contrast, \ourmethod{} calibrates noise to the contribution of individual updates (see Section~\ref{sec:privacy_analysis}). The signal-to-noise-ratio for the model updates is thus worse for \ourmethod{}. Secondly, in \ourmethod{} we have to clip client updates more aggressively to account for the privacy loss overhead incurred from the REC compression (roughly double for each iteration compared to Gaussian mechanism). This can be mitigated in larger federations, since the clipping can be reduced based on stronger privacy amplification for the central model of DP. For example, observe the StackOverflow experiment, where the accuracy delta between \ourmethod{} and \dpfedavg{} is smaller. Furthermore, it is precisely in those cases that reducing the communication cost is important from a practical perspective. When we target a \emph{specific accuracy} within the reach of both \ourmethod{} and \dpfedavg{}, we compress between $8.4$x (FEMNIST) to $1705$x (MNIST), at the additional cost of $2$ to $2.4$ in $\varepsilon$, relative to \dpfedavg{}.


\paragraph{Comparison with local DP guarantees}
The nature of the \ourmethod{} privacy mechanism requires calibrating noise to individual client updates rather than their contribution to the aggregate. This property warrants a different kind of comparison: equalizing local guarantees for each individual update (\emph{i.e.}, as seen when the secrecy of the sample in client sampling is not preserved). We use our non-i.i.d. FEMNIST setting with $1.5$k rounds and tune the noise of \dpfedavg{} such that a single client update, without any privacy amplification, has the same $\varepsilon_{\text{local}}$ guarantee. When training \dpfedavg{} with a local-DP guarantee that \ourmethod{} obtains when targeting central-DP with $\varepsilon = 3$,  we see that \dpfedavg{} obtains $68.9\%$ accuracy, whereas \ourmethod{} gets $63.4\%$. On a setting where we target the local-DP guarantee that \ourmethod{} gets when aiming for central-DP with $\varepsilon = 1$, \dpfedavg{} achieves $60.1\%$ accuracy compared to \ourmethod{}'s $57.4\%$. In both cases, \ourmethod{} achieves an overall compression rate of $72.5$x with $7$-bits per tensor, while losing $2.7\%$ to $5.5\%$ in accuracy compared to \dpfedavg{} (depending on the privacy target) due to more aggressive clipping. It is also worth noting that the performance delta relative to the results shown in Table~\ref{tab:acc_comm_res} is smaller, highlighting the negative effects of calibrating the noise to an ``aggregate'' of a single client.


\begin{wrapfigure}[16]{R}{0.36\textwidth}
    \vspace{-1em}
    \centering
    \includegraphics[width=0.36\textwidth]{figures/bit_ablation_femnist.png}
    \caption{Effect of the bit-width on model performance with \ourmethod{} for clipping  targeting $\varepsilon = 3$ after $1.5$k rounds. The ``no-compression'' variant communicates a random sample directly from $q_{\bs{\phi}}^{(t)}$ instead of compressing it via \ourmethod{}.}
    \label{fig:bitwidth_ablation}
\end{wrapfigure}

\paragraph{Compressibility of differentially private updates} As we noted in Section~\ref{sec:privacy_analysis}, differential privacy has a positive interplay with the \rec{} compression scheme. DP upper-bounds the R\'enyi divergence for any order $\lambda$ between the proposal distribution $p_{\bs{\theta}}^{(t)}$ and the model update distribution $q_{\bs{\phi}}^{(t)}$ and, according to lemma~\ref{the:Theorem2}, this limits the maximum bitrate $b$ of information to be communicated. In order to empirically verify this claim, we consider the non-i.i.d. FEMNIST classification with \ourmethod{}, and hyperparameters that target a model with $\varepsilon = 3$ after $1.5$k rounds. We then maintain the same bound on R\'enyi divergence and vary the number of bits per tensor from $4$ to $7$. We also include a variant without compression, which directly communicates a random sample from the clipped update distribution $q_{\bs{\phi}}^{(t)}$. 
The results appear to verify our claim and can be seen in Figure~\ref{fig:bitwidth_ablation}. After $4$ bits, we see very small improvements with adding additional bits and, with $7$ bits, the performance is very similar to the uncompressed baseline.

==> ICLR 2022/sections/intro.tex <==
\section{Introduction}
\label{sec:introduction}
The performance of modern neural-network-based machine learning models scales exceptionally well with the amount of data that they are trained on \citep{kaplan2020scaling,henighan2020scaling}. At the same time, industry \citep{flocwebsite}, legislators \citep{dwork2019differential,voigt2017eu} and consumers \citep{flurryblog} have become more conscious about the need to protect the privacy of the data that might be used in training such models. Federated learning (FL) describes a machine learning principle that enables learning on decentralized data by computing updates on-device. Instead of sending its data to a central location, a ``client'' in a federation of devices sends model updates computed on its data to the central server. Such an approach to learning from decentralized data promises to unlock the computing capabilities of billions of edge devices, enable personalized models and new applications in \textit{e.g.} healthcare due to the inherently more private nature of the approach. 

On the other hand, the federated paradigm brings challenges along many dimensions such as learning from non-i.i.d. data, resource-constrained devices, heterogeneous compute and communication capabilities, questions of fairness and representation, as well as the focus of our paper: communication overhead and characterization of privacy. Neural network training requires many passes over the data, resulting in repeated transfer of the model and updates between the server and the clients, potentially making communication a primary bottleneck~\citep{kairouz2019advances,wang2021field}. Compressing updates is an active area of research in FL and an essential step in ``untethering'' edge devices from WiFi. 
Moreover, while FL is intuitively more private through keeping data on-device, client updates have been shown to reveal sensitive information, even allowing to reconstruct a client's training data~\citep{geiping2020inverting}. To truly protect client privacy, a more rigorous mathematical notion of Differential Privacy (DP) is widely adopted as the de-facto standard in FL. More specifically, DP for FL is usually defined at a client-level, which provides plausible deniability of an individual client's contribution to the federated model. 
Both aspects of FL, communication efficiency and differential privacy, have been extensively studied in separation. Effective combination of the two, however, is an open problem and an active area of research \citep{kairouz2021distributed,chen2021breaking,girgis2020shuffled}. Some methods offer very limited compression capabilities for comparable utility \citep{kairouz2021distributed}, whereas others \citep{girgis2020shuffled} offer significant compression but require additional compromises, due to a looser privacy composition. 

In this work, we present \emph{Differentially Private Relative Entropy Coding} (\ourmethod{}), a unified approach to jointly tackle privacy and communication efficiency. \ourmethod{} makes use of the information-limiting constraints of DP to encode the client updates in FL with extremely short messages.
First, we build our method based on compression without quantization; namely, the lossy variant of Relative Entropy Coding (REC), recently proposed by \citet{flamich2020compressing}. Second, we show that it can be modified to satisfy DP, and we provide a proof of its privacy guarantees along with the appropriate accounting technique. Third, we run extensive evaluation on $4$ datasets and $3$ types of models to demonstrate that our algorithm achieves extreme compression of client-to-server updates (down to $7$ bits \textit{per tensor}) at privacy levels $\varepsilon < 1$ with a small impact on utility ($<6.5\%$ accuracy reduction on FEMNIST compared to \dpfedavg{}). Additionally, we show how to reduce server-to-client communication by sending a history of updates accumulated since the client's last participation.

==> ICLR 2022/sections/method.tex <==
\section{\ourmethod{} for private and efficient communication in FL}
Federated learning has been described by \citet{mcmahan2016communication} in the form of the \fedavg{} algorithm. At each communication round $t$, the server sends the current model parameters $\bv{w}^{(t)}$ to a subset $S^{(t)}$ of all clients $S$. Each chosen client $s$ updates the server-provided model $\bv{w}^{(t)}$, \emph{e.g.}, via stochastic gradient descent, to better fit its local dataset $D_s=\{d_{si}\}_{i=1}^{N_s}$ with a given loss function
\begin{align}
    \mathcal{L}_s(\mathcal{D}_s, \bv{w}) := \frac{1}{N_s}\sum_{i=1}^{N_s} L(d_{si}, \bv{w}).
\end{align}
After $E$ epochs of optimization on the local dataset, the client-side optimization procedure results in an updated model $\bv{w}^{(t)}_s$, based on which the client computes its update to the global model
\begin{align}
    \label{eq:fedavg_client_delta}
    \bs{\Delta}^{(t)}_s = \bv{w}^{(t)}_s - \bv{w}^{(t)};
\end{align}
and sends it to the server. The server then aggregates client-specific updates to get the new global model
$
    \bv{w}^{(t+1)} =\bv{w}^{(t)} + \frac{1}{|S^{(t)}|}\sum_s \bs{\Delta}^{(t)}_s = \frac{1}{|S^{(t)}|}\sum_s \bv{w}^{(t)}_s.
$
Outside the context of differential privacy, client updates are usually weighted by the size $N_s$ of the local dataset. A generalization of this server-side scheme \citep{reddi2020adaptive} interprets $\frac{1}{|S^{(t)}|}\sum_{s \in S^{(t)}} \bs{\Delta}^{(t)}_s$ as a ``gradient'' for the server-side model and introduces more advanced updating schemes, such as Adam \citep{kingma2014adam}. 

Federated training involves repeated communication of model updates from clients to the server and vice versa. These updates can reveal sensitive information about the client data, so there is a need for formal privacy guarantees. The total communication cost can be significant, thus constraining FL to the use of unmetered channels, such as WiFi. Hence, compressing the update messages in a privacy-preserving way plays an important role in moving FL to a truly mobile use-case. In the following sections, we first describe the lossy version of Relative Entropy Coding (REC) \citep{flamich2020compressing}, then show how to extend it to the FL scenario before discussing it in the context of differential privacy. Finally, we show how \ourmethod{} can be used to additionally compress server-to-client messages.

\subsection{REC for efficient communication}
\label{sec:compression_general}
Lossy REC, and its predecessor minimal random code learning (MIRACLE) \citep{havasi2018minimal}, have been originally proposed as a way to compress a random sample $\bv{w}$ from a distribution $q_{\bs{\phi}}(\bv{w})$ parameterized with $\bs{\phi}$, \emph{i.e.}, $\bv{w} \sim q_{\bs{\phi}}(\bv{w})$, by using information that is ``shared'' between the sender and the receiver. 
This information is given in terms of a shared prior distribution $p_{\bs{\theta}}(\bv{w})$ with parameters $\bs{\theta}$ along with a shared random seed $R$. 
The sender proceeds by generating $K$ independent random samples, $\bv{w}_1, \dots,\bv{w}_K$, from the prior distribution $p_{\bs{\theta}}(\bv{w})$ according to the random seed $R$. 
Subsequently, it forms a categorical distribution $\tilde{q}_{\bs{\pi}}(\bv{w}_{1:K})$ over the $K$ samples with the probability of each sample being proportional to the likelihood ratio $\pi_k \propto q_{\bs{\phi}}(\bv{w} = \bv{w}_k)/p_{\bs{\theta}}(\bv{w} = \bv{w}_k)$. Finally, it draws a random sample $\bv{w}_{k^*}$ from $\tilde{q}_{\bs{\pi}}(\bv{w}_{1:K})$, corresponding to the $k^*$'th sample drawn from the shared prior. The sender can then communicate to the receiver the \textit{index} $k^*$ with $\log_2 K$ bits. On the receiver side, $\bv{w}_{k^*}$ can be reconstructed by initializing the random number generator with $R$ and sampling the first $k^*$ samples from $p_{\bs{\theta}}(\bv{w})$. These procedures are described in Algorithms~\ref{alg:miracle_encode} and ~\ref{alg:miracle_decode}. 

\citet{havasi2018minimal} set $K$ to the exponential of the Kullback-Leibler (KL) divergence of $q_{\bs{\phi}}(\bv{w})$ to the prior $p_{\bs{\theta}}(\bv{w})$  with an extra constant $c$, \emph{i.e.}, $K = \exp(\text{KL}(q_{\bs{\phi}}(\bv{w}) || p_{\bs{\theta}}(\bv{w})) + c)$. In this case, the message length is at least $\mathcal{O}(\text{KL}(q_{\bs{\phi}}(\bv{w}) || p_{\bs{\theta}}(\bv{w})))$. This can be theoretically motivated based on the work by~\citet{harsha2007communication}; when the sender and the receiver share a source of randomness, under some assumptions, this $\text{KL}$ divergence is a lower bound on the expected message length~\citep{flamich2020compressing}. This brings forth an intuitive notion of compression that connects the compression rate with the amount of additional information encoded in $q_{\bs{\phi}}(\bv{w})$ relative to the information in $p_{\bs{\theta}}(\bv{w})$; the smaller the amount of extra information the shorter the message length will be and, in the extreme case where $q_{\bs{\phi}}(\bv{w}) = p_{\bs{\theta}}(\bv{w})$, the message length will be $\mathcal{O}(1)$. Of course, achieving this efficiency is meaningless if the bias of this procedure is high; fortunately, \citet{havasi2018minimal} show that for appropriate values of $c$ and under mild assumptions, the bias, namely $|\mathbb{E}_{\tilde{q}_{\bs{\pi}}(\bv{w}_{1:K})}[f] - \mathbb{E}_{q_{\bs{\phi}}(\bv{w})}[f]|$ for arbitrary functions $f$, can be sufficiently small. In all of our subsequent discussions, we parametrize $K$ as a function of a binary bit-width $b$, \emph{i.e.}, $K=2^b$, and treat $b$ as the hyperparameter.

\begin{figure}[t]
\begin{minipage}[t]{0.48\textwidth}
\vspace{-\baselineskip}
\begin{algorithm}[H]
\centering
\caption{The sender-side algorithm for lossy REC with the shared random seed $R$, the shared prior $p_{\bs{\theta}}(\bv{w})$ and the number of prior samples $K$.}\label{alg:miracle_encode}
\begin{algorithmic}
% \Function{Server}{}
\State Set state of pseudo-RNG to $R$
\State Draw $\bv{w}_1, \dots, \bv{w}_K \stackrel{\text{i.i.d.}}{\sim} p_{\bs{\theta}}(\bv{w})$
\State $\alpha_k \gets q_{\bs{\phi}}(\bv{w} = \bv{w}_k)/p_{\bs{\theta}}(\bv{w} = \bv{w}_k)$
\State $\pi_k \gets \alpha_k /\sum_j \alpha_j$
\State $\bv{w}_{k^*} \sim \tilde{q}_{\bs{\pi}}(\bv{w}_{1:K})$\\
\Return $k^*$ encoded with $\log_2 K$ bits
\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\vspace{-\baselineskip}
\begin{algorithm}[H]
\centering
\caption{The receiver-side algorithm for lossy REC.}\label{alg:miracle_decode}
\begin{algorithmic}
\State Receive $k^*$ from the sender
\State Set state of pseudo-RNG to $R$
\State Draw $\bv{w}_1, \dots, \bv{w}_{k^*} \stackrel{\text{i.i.d.}}{\sim} p_{\bs{\theta}}(\bv{w})$
\State Use $\bv{w}_{k^*}$ for downstream task
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{figure}

\subsection{REC for efficient communication in FL}
\label{sec:compression}
We can adapt this procedure to FL by appropriately choosing distributions over client-to-server messages (model updates), $q^{(t)}_{\bs{\phi}_s}(\bs{\Delta}^{(t)}_s)$ , along with the prior distribution $p^{(t)}_{\bs{\theta}}(\bs{\Delta}^{(t)}_s)$ on each round $t$:
\begin{align}
\label{eq:define_p_q}
    p ^{(t)}_{\bs{\theta}}(\bs{\Delta}^{(t)}_s) := \mathcal{N}(\bs{\Delta}^{(t)}_s | \bv{0}, \sigma^2\bv{I}), \qquad q^{(t)}_{\bs{\phi}_s}(\bs{\Delta}^{(t)}_s) := \mathcal{N}(\bs{\Delta}^{(t)}_s | \bv{w}^{(t)}_s - \bv{w}^{(t)}, \sigma^2\bv{I}),
\end{align}
\emph{i.e.}, for the prior we use a Gaussian distribution centered at zero with appropriately chosen $\sigma$ and for the message distribution we opt for a Gaussian with the same standard deviation centered at the model update.
The form of $q$ is chosen to provide a plug-in solution to potentially resource constrained devices, as well as to readily satisfy the differential privacy constrains discussed in Section \ref{sec:privacy_mechanism}.
Note that, as opposed to the \fedavg{} client update definition in \eqref{eq:fedavg_client_delta}, here we consider $\bs{\Delta}^{(t)}_s$ to be a random variable and the difference $\bv{w}^{(t)}_s - \bv{w}^{(t)}$ to be the mean of the client-update distribution $q$ over $\bs{\Delta}^{(t)}_s$.

Let us now see how communication efficiency is realized in the FL pipeline. The length of the message will be a function of how much ``extra'' information about the local dataset $D_s$ is encoded in $\bv{w}^{(t)}_{s}$, measured by KL divergence. As we show later, this has a nice interplay with DP: the DP constraints bound the amount of information encoded in each update, resulting in highly compressible messages. It is also worth noting that this procedure can be done parameter-wise (\emph{i.e.}, communicate $\log_2 K$ bits per parameter), layer-wise ($\log_2 K$ bits for each layer in the network) or even network-wise ($\log_2 K$ bits in total). Any arbitrary intermediate vector size is also possible. This is done by splitting $\bs{\Delta}^{(t)}_s$ into $M$ independent groups (which is possible due to our assumption of factorial distributions over the dimensions of the vector) and applying compression independently to each group (see also Theorem~\ref{thm:Theorem3}). If we have many groups (\textit{e.g.}, when we perform per-parameter compression), we can boost the compression even further by entropy coding the indices with their empirical distribution.


\subsection{Private \& efficient communication for FL with \ourmethod{}}
\label{sec:privacy_mechanism}
In order to make the compression procedure described in Section~\ref{sec:compression} differentially private, we need to bound the sensitivity of the mechanism and quantify the noise inherent to it. Similarly to \dpfedavg{}, bounding the sensitivity consists of clipping the norm of client updates $\bv{w}^{(t)}_s - \bv{w}^{(t)}$. In the context of REC, this means that the client message distribution $q_{\bs{\phi}}^{(t)}$ cannot be too different from the server prior $p_{\bs{\theta}}^{(t)}$ in any given round $t$. After this step, instead of explicitly injecting additional noise to the updates, we make use of the fact that the procedure in itself is stochastic. Two sources of randomness play a role in each round $t$: (1) drawing $K$ samples from the prior $p_{\bs{\theta}}^{(t)}$; (2) drawing an update from the importance sampling distribution $\tilde{q}_{\bs{\pi}}^{(t)}$. We coin the name Differentially-Private Relative Entropy Coding (\ourmethod{}) for the resulting mechanism, outlined in Algorithms~\ref{alg:fedpc_encode} and ~\ref{alg:fedpc_decode}.

\begin{minipage}[t]{0.6\textwidth}
\vspace{-\baselineskip}
\begin{algorithm}[H]
\centering
\caption{The client-side algorithm for \ourmethod{} at a given round $t$. $R_s^{(t)}$ is the client-chosen shared random seed, $\bv{w}^{(t)}$ is the server model, $\bv{w}^{(t)}_s$ is the fine-tuned model of client $s$, $K$ is the number of prior samples, $C$ is the clipping threshold and $\sigma$ is the prior standard deviation.}\label{alg:fedpc_encode}
\begin{algorithmic}
\State $R_s^{(t)} \gets$ choose and set client-specific seed for round $t$
\State $\bs{\phi}^{(t)}_s \gets \bv{w}^{(t)}_s - \bv{w}^{(t)}$
\State $\bs{\Delta}_1, \dots, \bs{\Delta}_K \stackrel{\text{i.i.d.}}{\sim} \mathcal{N}(\bs{\Delta}^{(t)}_s| \bv{0}, \sigma^2\bv{I})$
\State $\hat{\bs{\phi}}^{(t)}_s = \bs{\phi}^{(t)}_s \min(1, C / \|\bs{\phi}^{(t)}_s\|_2)$
\State $\alpha_k \gets \mathcal{N}(\bs{\Delta}^{(t)}_s = \bs{\Delta}_k| \hat{\bs{\phi}}^{(t)}_s, \sigma^2\bv{I})/\mathcal{N}(\bs{\Delta}^{(t)}_s = \bs{\Delta}_k| \bs{0}, \sigma^2\bv{I})$
\State $\pi_k \gets \alpha_k /\sum_j \alpha_j$
\State $\bs{\Delta}_{k^*} \sim \tilde{q}^{(t)}_{\bs{\pi}}(\bs{\Delta}_{1:K})$\\
\Return $k^*$ encoded with $\log_2 K$ bits, $R_s^{(t)}$
\end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill
\begin{minipage}[t]{0.38\textwidth}
\vspace{-\baselineskip}
\begin{algorithm}[H]
\centering
\caption{The server side algorithm for \ourmethod{}.}\label{alg:fedpc_decode}
\begin{algorithmic}
\State Receive $k^*, R_s^{(t)}$ from client $s$
\State Set state of pseudo-RNG to $R_s^{(t)}$
\State $\bs{\Delta}_1, \dots, \bs{\Delta}_{k^*} \stackrel{\text{i.i.d.}}{\sim} \mathcal{N}(\bs{\Delta}^{(t)}_s| \bv{0}, \sigma^2\bv{I})$
\State Use $\bs{\Delta}_{k^*}$ for downstream task
\end{algorithmic}
\end{algorithm}
\end{minipage}

Finally, to prove that \ourmethod{} is differentially private and calculate the corresponding $\varepsilon, \delta$, we build upon prior work in privacy accounting for ML and FL; particularly, on R\'enyi differential privacy (RDP)~\citep{mironov2017renyi} and the moments accountant~\citep{abadi2016deep}. Our analysis in the next section follows the established approach based on tail bounds of the privacy loss random variable, addressing such important differences as two sources of randomness and non-Gaussianity of $\tilde{q}_{\bs{\pi}}^{(t)}$.
Additional discussion on other aspects of our method can be found in Appendices~\ref{sec:app_additional_discussion} and~\ref{sec:app_private_mean_estimation}.

\subsection{Privacy Analysis of \ourmethod{}}
\label{sec:privacy_analysis}
A possible avenue to analyze privacy for \ourmethod{} is to derive DP bounds  relying on Theorem 3.2 of \citet{havasi2018minimal}. However, obtaining reasonable guarantees can be challenging, as the probability bound in~\citep[Theorem 3.2]{havasi2018minimal} has to be incorporated in $\delta$ and it is at least $e^{-0.125 \ln K}$. As such, a fairly common value $\delta = 10^{-5}$ would require ${\scriptscriptstyle~^\sim} e^{92}$ samples from the prior. To overcome this issue, we consider an importance sampling bound by \citet[Section~2.2]{agapiou2017importance}. It scales (inversely) linearly with the number of samples, helping for smaller sample sizes.

Let us restate the bound for completeness. For some test function $\zeta$, one can characterize the bound between the true expectation and the importance sampling estimate in the following way:
\begin{align}
    &\sup_{|\zeta| < 1} \left| \mathbb{E} \left[ \mu^N (\zeta) - \mu(\zeta) \right] \right| \leq \frac{12}{K} e^{\mathcal{D}_2(q_{\bs{\phi}} || p_{\theta})}, \label{eq:sup_ex_bound}
\end{align}
where $K$ is the number of samples, $\mu^N(\cdot) = \mathbb{E}_{\tilde{q}_{\bs{\pi}}}[\cdot]$, $\mu(\cdot) = \mathbb{E}_{q_{\bs{\phi}}}[\cdot]$ and $\mathcal{D}_2 (\cdot||\cdot)$ denotes the R\'enyi divergence of order $2$ between the target $q_{\bs{\phi}}$ and the proposal $p_{\bs{\theta}}$. Our choice of $\zeta$ (\emph{cf.} Appendix \ref{sec:proof_of_main_theorem}) guarantees $|\zeta| < 1$ for any input and enables the use of this bound.

Theorem~\ref{the:Theorem1} summarizes our main theoretical result. It enables \ourmethod{} to combine the server-side privacy accounting in the central model of DP with extreme model update compression, while allowing clients to privatize their updates locally and protect against an honest-but-curious server.
\begin{theorem}
\label{the:Theorem1}
After $T$ rounds, with the client-to-server bitrate $b$, \ourmethod{} is differentially private with 
\begin{align*}
    \delta \leq \min_\lambda e^{-\lambda\varepsilon} \prod_{t=1}^T e^{2\lambda c_{\lambda+1}^{(t)}} + \frac{12}{2^b} \sum_{t=1}^{T} e^{c_2^{(t)}},
\end{align*}
where the constant $c_\lambda^{(t)} \geq \max \left\{ \mathcal{D}_\lambda \left(q_{\bs{\phi}}^{(t)} || p_{\bs{\theta}}^{(t)} \right), \mathcal{D}_\lambda \left(p_{\bs{\theta}}^{(t)} || q_{\bs{\phi}}^{(t)} \right) \right\}$ is the upper bound on R\'enyi divergences of order $\lambda$ between the client model update distribution $q_{\bs{\phi}}^{(t)}$ and the server prior $p_{\bs{\theta}}^{(t)}$ in any given round $t$ (in both directions).
\end{theorem}
\begin{proof}
See Appendix \ref{sec:proof_of_main_theorem}.
\end{proof}

An attentive reader may notice a strong resemblance between Theorem~\ref{the:Theorem1} and the moments accountant~\citep{abadi2016deep} and R\'enyi DP~\citep{mironov2017renyi} results. Indeed, it turns out that the \ourmethod{} compression procedure yields the privacy loss that can be bound by almost the double of the normal continuous Gaussian mechanism loss, plus a small overhead, and composed in a very similar manner.

\textbf{Shared random seed}~ Prior work relying on shared random seeds has been shown to be vulnerable to attacks due to the possibility of ``inverting'' the noise~\citep{kairouz2021distributed}. \ourmethod{} is not susceptible to this for two reasons. First, the randomness of the method comes from two sources instead of one, and knowing one seed does not permit to fully reconstruct the un-noised sample. In our guarantee, $\delta$ corresponds to the probability of the mechanism failure w.r.t. both sources of randomness, making it as secure as the standard Gaussian mechanism even when one of the seeds is shared. However, this alone is not sufficient because the shared seed $R$ could be manipulated to generate a set of samples on which to encode the update such that the guarantee would not hold (\emph{e.g.}, in the tails of the privacy loss distribution). Hence, we add the second line of defense as we shift the task of picking $R$ to a client, who then transmits the seed along with the index $k^*$ for decoding. This way, neither the server nor any other entity can manipulate the seed to break the privacy guarantee.

\textbf{Privacy amplification}~
Like many recent approaches, including~\citep{kairouz2021distributed}, \ourmethod{} can be seen as a hybrid method, privatizing updates locally and providing an amplified central guarantee. A key difference, however, is that our method does not calibrate noise to the aggregate. Namely, the scale of noise and the guarantee do not depend on whether a thousand, a hundred, or just one client is sampled in a round. This is due to non-additive nature of our mechanism, which does not let us easily benefit from the variance reduction as the Gaussian mechanism does. As a result, we always calibrate to an ``aggregate'' of one client. While this property increases the necessary noise, it has an upside of allowing stronger privacy amplification. Substituting the typical sampling \emph{without replacement} by sampling \emph{with replacement}, we can use the amplification factor of $1/|S|$ while accounting for $T|S'|$ rounds, instead of $|S'|/|S|$ while accounting for $T$ rounds, and obtain a tighter overall guarantee.

\textbf{Secure aggregation}~
One of the considerations in FL is that the server might be honest-but-curious rather than fully trusted. In \dpfedavg{}~\citep{mcmahan2017learning}, the noise addition is delegated to the server, and thus, secure aggregation~\citep{bonawitz2017practical} is necessary to prevent the server from receiving client updates in the clear. \ddgauss{}~\citep{kairouz2021distributed} and analogous methods mitigate this problem by shifting the noise addition to the client side, but still use secure aggregation for the reasons stated in the previous paragraph: noise is calibrated to the aggregate and may be insufficient to protect some clients. In \ourmethod{}, because of the noise calibration to individual updates, we believe that the provided local guarantee (which can be computed by removing subsampling amplification) is sufficient against non-malicious servers. To further boost privacy protection, an important future work direction is integrating the \ourmethod{} compression scheme with secure aggregation.

\textbf{Interplay of privacy and compression}~ Theorem \ref{the:Theorem1} relates privacy to our compression scheme in an intuitive manner. In order to get meaningful privacy guarantees, we have to bound the R\'enyi divergence in any given round $t$ for any $\lambda \geq 1$, which limits the amount of information encoded in $q_{\bs{\phi}}^{(t)}$ relative to $p_{\bs{\theta}}^{(t)}$. As a result, enforcing DP guarantees also implies that our scheme will have highly compressible messages. We formalize this interplay in the following lemma.
    
\begin{lemma}
\label{the:Theorem2}
Consider compressing the expected value of $\zeta$ under the $q_{\phi_s}(\bs{\Delta}_s)$ at \eqref{eq:define_p_q}, and let $\xi$ be a desired average compression bias of \rec{} for $\zeta$. To achieve this target, a sufficient bitrate $b$ is at most
\begin{align*}
    b \leq \log_{2}{12} + \frac{1}{\log{2}}\mathcal{D}_2\left(q_{\bs{\phi}_s} || p_{\theta}\right) - \log_{2}{\frac{\xi}{G}},
\end{align*}
where $|\zeta| \leq G$ and $\mathcal{D}_2\left(q_{\bs{\phi}_s} || p_{\theta}\right)$, and thus the maximum bitrate $b$, is controlled by the chosen $(\varepsilon, \delta)$.
\end{lemma}
\begin{proof}
The proof follows from \eqref{eq:sup_ex_bound}, by setting $K=2^b$, rearranging the terms and adjusting for $G$.
\end{proof}
We also verify the claim empirically (Figure~\ref{fig:bitwidth_ablation}), fixing the bound on the R\'enyi divergence and showing that the performance with extreme compression (\emph{i.e.}, $7$ bits$/$tensor) and no compression is similar. 
Finally, to confirm that various granularity of compression (per-parameter, per-layer, per-network, etc.) does not interfere with our privacy analysis, we introduce and prove the following theorem.

\begin{theorem}[Compression-by-parts]
\label{thm:Theorem3}
Expectation of an arbitrary function $\zeta(\bs{\Delta}^{[1]}, \ldots, \bs{\Delta}^{[M]})$ over the importance sampling distributions $q_{\bs{\pi}}^{[1]}, \ldots, q_{\bs{\pi}}^{[M]}$, built for $M$ non-intersecting parameter groups independently, is equivalent to the expectation over the joint distribution $q_{\bs{\pi}}$ built on $2^{\sum_{i=1}^{M}b_i}$ samples:
\begin{align*}
    \mathbb{E}_{\bs{\Delta}^{[1]} \sim q_{\bs{\pi}}^{[1]}} \left[ \ldots \mathbb{E}_{\bs{\Delta}^{[M]} \sim q_{\bs{\pi}}^{[M]}} \left[ \zeta(\bs{\Delta}^{[1]}, \ldots, \bs{\Delta}^{[M]}) \right] \ldots \right] = \mathbb{E}_{\bs{\Delta}^{[1:M]} \sim q_{\bs{\pi}}} \left[ \zeta(\bs{\Delta}^{[1:M]}) \right].
\end{align*}
\end{theorem}
\begin{proof}
See Appendix \ref{sec:compression_by_parts}.
\end{proof}

\subsection{Compressing server-to-client messages}
\label{sec:compressingServerToClient}
The compression procedure described in Section \ref{sec:compression} is a specific example of (stochastic) vector quantization where the shared codebook is determined by a shared random seed. Here we show how the principle of communicating indices into such a shared codebook additionally allows for the compression of the server-to-client communication. Instead of sending the full server-side model to a specific client, the server can choose to collect all updates to the global model in-between two subsequent rounds that the client participates in. Based on this history of codebook indices, the client can deterministically reconstruct the current state of the server model before beginning local optimization. Clearly, the expected length of the history is proportional to the total number of clients and the amount of client subsampling we perform during training. At the beginning of a round, the server can therefore compare the bit-size of the history and choose to send the full-precision model $\bv{w}^{(t)}$ instead. 
Taking a model with $1k$ parameters as an example, a single uncompressed model update is approximately equal to $4k$ communicated indices when using $8$-bit codebook compression of the whole model. 
Crucially, compressing server-to-client messages this way has no influence on the DP nature of \ourmethod{} since the local model of DP ensures privacy of client information (and the stronger central guarantee applies as long as the secrecy of the sample is preserved within the updates history).

For clients participating in their first round of training, the first seed without accompanying indices can be understood as seeding the random initialization of the server-side model. Algorithms \ref{alg:miracle_server_to_client_compression} and \ref{alg:miracle_server_to_client_decode} (in Appendix \ref{sec:AppStoCcompression}) describe this scheme. It is important to note that the client-side update rule must be equal to the server-side update rule, \emph{i.e.} in generalized \fedavg{} \citep{reddi2020adaptive} it might be necessary to additionally send the optimizer state when sending the current global model $\bv{w}^{(t)}$.




==> ICLR 2022/sections/related.tex <==
\section{Related work}
\label{sec:related_work}
The privacy promise of federated learning relies heavily on the use of additional techniques, such as differential privacy and secure multi-party computation, to provide rigorous theoretical guarantees. Without these techniques, FL has been shown to be vulnerable to attacks~\citep{geiping2020inverting} and unintended leakage of sensitive information~\citep{thakkar2020understanding}. One of the main open challenges is to reduce the communication cost while preserving DP guarantees~\citep{kairouz2019advances}.

\citet{mcmahan2017learning} outlined \dpfedavg{}, which has since been the staple of DP federated learning. In this default scheme, clients clip norms of their updates before submitting them to the server (preferably, using a secure aggregation protocol~\citep{bonawitz2017practical}). The server then completes the DP mechanism by adding Gaussian noise to the aggregate of multiple clients. Without secure aggregation, this method allows clients to compress their updates and reduce communication, but becomes vulnerable to a malicious or honest-but-curious server. One could use the local model of DP~\citep{dwork2014algorithmic} instead of the central model to address this issue: clients would add noise locally before sending the updates. But this leads to a pronounced drop in accuracy due to the larger scale of noise necessary in the local model~\citep{kairouz2019advances}. The few existing examples that use the local model operate on very large numbers of clients and updates~\citep{pihur2018differentially}.

To overcome this problem of excessive noise, researchers are increasingly looking in the direction of hybrid solutions~\citep{shi2011privacy,rastogi2010differentially,agarwal2018cpsgd,truex2019hybrid}. The key idea of these techniques is to reduce the variance of the locally added noise by taking into account the larger global number of clients and accounting DP in the central model. Since the smaller noise variance is insufficient to protect individual updates, secure aggregation is necessary for these methods. In this context, the local noise distributions have to be discrete, such that their sum after secure aggregation is also discrete and is of known shape, allowing the server to compute guarantees centrally. As a result, until recently, most of these methods relied on the binomial distribution. Compared to the traditional Gaussian mechanisms, it is at a disadvantage because it does not yield Renyi or concentrated DP, and thus cannot benefit from tighter adaptive composition and amplification through sampling, which is particularly important in ML applications~\citep{kairouz2021distributed}. \citet{kairouz2021distributed} presented a novel analysis of the discrete Gaussian mechanism~\citep{canonne2020discrete} in terms of concentrated DP. Their mechanism, named Discrete Distributed Gaussian (\ddgauss{}), is adapted to the context of FL, can provide accuracy comparable to the centralized Gaussian mechanism, and enables parameter-wise quantization. However, at higher compression rates (\emph{e.g.}, $12$ bits per parameter), \ddgauss{} fails to train a model for reasonable $\varepsilon$ values.

Finally, there is recent work featuring extreme compression rates for DP algorithms, bearing a resemblance to our solution. \citet{girgis2020shuffled} proposed to use a locally private mechanism along with a secure shuffler to communicate models one (privatized) parameter at a time. It compresses client messages to $\log d$ bits for a model of $d$ parameters. This approach, however, seems to require a large number of clients to participate in a single round ($10$k for their MNIST experiment), which is impractical in realistic scenarios and detrimental to the total communication cost (upload + download). 
\citet{chen2021breaking} achieve similarly high compression rates as~\citep{girgis2020shuffled}; however, they do not consider the context of federated learning but rather focus on frequency and mean estimation. As we did not have an FL baseline for \citep{chen2021breaking} and could not reliably reproduce the results of \citet{girgis2020shuffled}, we focused our comparison with these methods on mean estimation. Details can be found in Appendix~\ref{sec:app_private_mean_estimation}. In short, we find that the method of \cite{chen2021breaking} has an edge over \ourmethod{} if a good prior is lacking, making it preferable for low-information, ``one-shot'' scenarios, such as mean estimation. On the other hand, with a good prior (or one that is learned during training), \ourmethod{} performs better and thus is more appropriate in federated settings.



